Decision Procedures for Path Feasibility of String-Manipulating Programs with Complex Operations

The design and implementation of decision procedures for checking path feasibility in string-manipulating programs is an important problem, whose applications include symbolic execution and automated detection of cross-site scripting (XSS) vulnerabilities. A (symbolic) path is a finite sequence of assignments and assertions (i.e. without loops), and checking its feasibility amounts to determining the existence of inputs that yield a successful execution. We give two general semantic conditions which together ensure the decidability of path feasibility: (1) each assertion admits regular monadic decomposition, and (2) each assignment uses a (possibly nondeterministic) function whose inverse relation preserves regularity. We show these conditions are expressive since they are satisfied by a multitude of string operations. They also strictly subsume existing decidable string theories, and most existing benchmarks (e.g. most of Kaluza's, and all of SLOG's, Stranger's, and SLOTH's). We give a simple decision procedure and an extensible architecture of a string solver in that a user may easily incorporate his/her own string functions. We show the general fragment has a tight, but high complexity. To address this, we propose to allow only partial string functions (i.e., prohibit nondeterminism) in condition (2). When nondeterministic functions are needed, we also provide a syntactic fragment that provides a support of nondeterministic functions but can be reduced to an existing solver SLOTH. We provide an efficient implementation of our decision procedure for deterministic partial string functions in a new string solver OSTRICH. It provides built-in support for concatenation, reverse, functional transducers, and replaceall and provides a framework for extensibility to support further string functions. We demonstrate the efficacy of our new solver against other competitive solvers.

==> auto-sanitisation.tex <==
\smallskip
\noindent \textbf{Context-sensitive auto-sanitisation example.} %Transductions.}
%
%
%parametric transducers can model string functions required in \emph{context-sensitive
%	auto-sanitisation} in web templating systems \cite{SSS11}, e.g., Google Closure 
%\cite{Closure} and Handlebars \cite{Handlebars}. 
%
Web pages are often constructed using templating systems \cite{SSS11} such as Mustache.js or Google Closure.
Template HTML contains variables that are instantiated before the page is served.
A simple template is given in Figure~\ref{fig:closure}(\ref{fig:closure-eg}) with variables \linkvar\ and \linktextvar.
%A parametric transducer can instantiate the variables with runtime values using the variable parameters.
%However 
Templating systems may also provide a context-aware ``auto-escape'' feature.
That is, the contents of the replaced variable will be ``escaped'' so that special characters (or sequences) which may allow code injection are replaced with safe alternatives to avoid attack.
The escaping applied depends on the text surrounding the variable use.
%\mat{Changed above text to try and emphasize variables and context}

\zhilin{adapt the following example to demonstrate the use of transducers and replaceAll function}\zhilin{Could we have an example to demonstrate the use of transducers, replaceAll function and reverse function ?}

For example, if \linkvar\ had the value \mintinline{js}{javascript: alert(1337)}, clicking the link in the instantiated template would run the JavaScript code \mintinline{js}{alert(1337)}.
To avoid this, Closure wraps URLs beginning with \mintinline{html}{javascript:} in single quotes.
Providing the value \mintinline{html}{<script>alert(1337)</script>} to \linktextvar\ would have a similar effect, but this time Closure replaces \texttt{<} with \texttt{\&lt;} and \texttt{>} with \texttt{\&gt;}.
%
\begin{wrapfigure}{r}{0.8\textwidth}
\begin{center}
  %  \vspace*{-6ex}
\begin{minipage}{\linewidth}
\begin{enumerate}[(a)]
\item \label{fig:closure-eg}
\begin{minted}{html}
<a href="{$li}"> {$txt} </a>
\end{minted}
\item \label{fig:closure-tagged}
\begin{minted}{html}
<a href="[URL]javascript: alert(1337)[LRU]">
    [HTML]<script>alert(1337)</script>[LMTH] </a>
\end{minted}
\item \label{fig:closure-safe}
\begin{minted}{html}
<a href="'javascript: alert(1337)'">
    &lt;script&gt;alert(1337)&lt;/script&gt; </a>
\end{minted}
\end{enumerate}
\end{minipage}
\end{center}
%\vspace{-3ex}
\caption{\label{fig:closure}A simple template (\ref{fig:closure-eg}) with two transduction steps (\ref{fig:closure-tagged}, \ref{fig:closure-safe}).}
%\vspace{-5ex}
\end{wrapfigure}
A key point is that the safe transduction depends on the context of the variable:
the escaping in a URL context is different to that in an HTML context.
We can model this using two transducers.
The first transducer instantiates the variables, but surrounds them with markers to indicate that the text inside needs to be escaped
(Figure~\ref{fig:closure}(\ref{fig:closure-tagged}));
we use \urlstarttag, \urlendtag, \htmlstarttag, and \htmlendtag.
Since transducers are a generalisation of finite automata, they are able to identify contexts using regular languages. The second transducer then applies the appropriate safe transductions inside the markers.
For the URL context, values starting with \texttt{javascript:} will be quoted, while in HTML, instances of \texttt{<} and \texttt{>} are replaced by \texttt{\&lt;} and \texttt{\&gt;} respectively.
The result is shown in Figure~\ref{fig:closure}(\ref{fig:closure-safe}).

%\zhilin{Can I understand the example in the following way? The first transducer is in fact the composition of the following two assignments 
% $$x' := \replaceall(x, "\{\$li\}", [URL] y_{li} [LRL])$$ 
% and 
% $$x'' := \replaceall(x', "\{\$txt\}", [HTML]y_{txt}[LTMH]),$$ 
% where $x$ represents the input string, and $y_{li}, y_{txt}$ are parameters. The second transducer is in fat a non-parametric transducer to do the sanitisation. Strictly speaking, this demonstrates the necessity to have both $\replaceall$ function and finite-state transducers, but not exactly the necessity of parametric transducers. But of course, it is nice to have a single formalism where both $\replaceall$ and finite-state transducers can be captured.}
%
%\mat{
%    @Zhilin
%    The first replaceall needs to be a transducer because it is context-aware.
%    I.e. it uses the fact that \linkvar\ appears in a value of an href attribute to know that it needs to be sanitised like a URL rather than HTML.
%}

%\mat{
%    One might worry that identifying text starting with \texttt{javascript:} means the transudcer needs to keep a buffer of the input string, leading to large transducers.
%    In fact, we can avoid this by having the transducer non-deterministically guess that the following string will begin with \texttt{javascript:} and then verifying later that this was or was not the case.
%    Let me know if you think i should put a footnote about this.
%    It would also apply to contexts that need to see the text after the variable to confirm the (guessed) context is the right one.
%}





==> escapeString.tex <==
\begin{figure}
    \begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2.3cm,on grid,auto, initial text={}] 
    \node[state,initial,accepting] (q_0) {$q_0$}; 
%    \node[state] (q_1) [above right=of q_0] {$q_1$}; 
%    \node[state] (q_2) [below right=of q_0] {$q_2$}; 
    \path[->]
    (q_0) edge  [loop above] node {$\ell$/$\ell$} (q_0)
  	    edge  [loop right] node {\texttt{'}/\texttt{\textbackslash'}} (q_0)
          edge  [loop below] node {\texttt{"}/\texttt{\textbackslash"}} (q_0);
%          edge  [bend left] node [right] {\texttt{"}/\texttt{\textbackslash}} (q_2)
%    (q_1) edge  [bend left] node  {$\epsilon$/\texttt{'}} (q_0)
%    (q_2) edge  [bend left] node  {$\epsilon$/\texttt{"}} (q_0);
\end{tikzpicture}
    \end{center}
    \caption{
        A transducer that replaces every occurrence of \texttt{'} and
    \texttt{"} with, respectively, \texttt{\textbackslash '} and 
    \texttt{\textbackslash "}. Here,
    $\ell$ is every symbol in the alphabet that is neither 
    \texttt{'} nor \texttt{"}. \label{fig:escapeString}}
\end{figure}


==> expspace-macros.tex <==

% General
\newcommand\brac[1]{\left(#1\right)}
\newcommand\tup\brac

% \setcomp{ele}{comp} = { ele | comp }
\newcommand\setcomp[2]{\left\{{#1}\ \middle|\ {#2}\right\}}

% \lang{A} = L(A)
\newcommand\lang[1]{\mathcal{L}\mathord{\brac{#1}}}


% Tiling

\newcommand\width{\ell}
\newcommand\height{h}
\newcommand\hcons{H}
\newcommand\vcons{V}
\newcommand\tiles{T}
\newcommand\tile{t}
\newcommand\inittile{t_0}
\newcommand\fintile{t_f}
\newcommand\rowdelim{\#}

% Reduction
\newcommand\resetchar{!}
\newcommand\bit{b}

% \nbit[i][0] = 0_i, similarly for 1
\newcommand\nbit[2]{{#2}_{#1}}

% \repl{n}{0}{1} = $^1_{n,0} means if nth bit is 0, turn into a 1
\newcommand\repl[3]{\$^{#3}_{#1, #2}}
\newcommand\replall[1]{\$_{#1}}


==> extensions.tex <==
%!TEX root = main.tex

\section{Extensions}\label{sec-ext}

In this section, we consider the language $\strline$ extended with either integer assertions, character assertions, or $\indexof$ assertions, and show that while  in general each of such extensions leads to undecidability, the decidability holds for \strlineconcat, actually even with the same complexity. 
%\mat{Should $\concat$ be removed?}\zhilin{agree, since the undecidability result is stronger if stated for $\strline[\replaceall]$}
We will use variables of, in additional to the type $\str$, the Integer data type $\intnum$. A variable of type $\intnum$, usually referred to as an \emph{integer variable}, ranges over the set $\Nat$ of natural numbers. Recall that, in previous sections, we have used $x, y, z, \ldots$ to denote the variables of $\str$ type.  Hereafter we typically use $\mathfrak{l}, \mathfrak{m}, \mathfrak{n}, \ldots$ to denote the variables of $\intnum$. The
choice of omitting negative integers is for simplicity. Our
results can be easily extended to the case where $\intnum$ includes negative integers.

We begin by defining the kinds of assertions we will use to extend $\strline$.
First, we describe integer assertions, which express conditionals on the length or number of occurrences of symbols in words. 


\begin{definition}[Integer assertions] \label{def:intconst} 
	An integer assertion is of the form
	$\ASSERT{a_1t_1+\cdots+a_nt_n\leq d}$, 
where $a_1, \cdots, a_n,d\in \mathbb{Z}$ are  integer constants (represented in binary), and each \emph{term} $t_i$ is either 
	\begin{enumerate}
		\item an integer variable $\mathfrak{n}$;
		\item $|x|$ where $x$ is a  string variable; or 
		\item $|x|_a$ where $x$ is string variable and $a\in \Sigma$ is a constant letter.
	\end{enumerate}
Here, $|x|$ and $|x|_a$ denote the length of $x$ and the number of occurrences of $a$ in $x$, respectively. 
%
%An \emph{integer constraint} over $\Sigma$ is a Boolean combination of atomic integer constraints over $\Sigma$.
\end{definition}

Character assertions, on the other hand, allow to compare symbols from different strings. The formal definitions are given as follows. 

\begin{definition}[Character assertions]
	A \emph{character assertion}  is of the form $\ASSERT{x[t_1]=y[t_2]}$, where 
	\begin{itemize}
		\item $x$ and $y$ are either a string variable or a  string constant in $\Sigma^*$, and 
		\item $t_1$ and $t_2$ are either integer variables or  positive integer constants.
	\end{itemize} 
Here, the interpretation of $x[t_1]$ is the $t_1$-th letter of $x$. In case that $x$ does not have the $t_1$-th letter \emph{or} $y$ does not have the $t_2$-th letter, the constraint $x[t_1] = y[t_2]$ is false by convention.  
%Similarly for $y[t_2]$.
%\mat{What if $x$ doesn't have a $t_1$th letter?}\zhilin{how about this ?}
%	
%A \emph{character constraint} over $\Sigma$ is a Boolean combination of atomic character constraints over $\Sigma$. 
\end{definition}

We also consider the constraints involving the $\indexof$ function.

\begin{definition}[$\indexof$ assertions]
An {$\indexof$ assertion} is of the form $\ASSERT{t\ \mathfrak{o}\ \indexof(s_1, s_2)}$, where 
\begin{itemize}
\item $t$ is an integer variable, or a positive integer constant (recall that here we assume that the first position of a string is $1$), or the value $0$ (denoting that there is no occurrence of $s_1$ in $s_2$), 
\item $\mathfrak{o} \in \{\ge, \le\}$, and
%
\item  $s_1,s_2$ are either string variables or  string constants. 
\end{itemize}
We consider the \emph{first-occurrence} semantics of $\indexof$.  More specifically, $t \ge \indexof(s_1, s_2)$ holds if $t$ is no less than the first position in $s_2$ where $s_1$ occurs, similarly for $t \le \indexof(s_1, s_2)$.
%\mat{What if $s_1$ does not appear in $s_2$?}\zhilin{if $s_1$ does not appear in $s_2$, then $\indexof(s_1, s_2)=0$, as defined above.}
%
%An $\indexof$ constraint over $\Sigma$ is a Boolean combination of atomic $\indexof$ constraints over $\Sigma$.
\end{definition}

\begin{theorem}[\cite{CCHLW18}]
The path feasibility of \strlinefft{} extended with any of integer assertions, character assertions, or $\indexof$ assertions, is undecidable.
\end{theorem}

\begin{theorem}
The path feasibility of \strlineconcat{} extended with integer assertions, character assertions, and $\indexof$ assertions, is \expspace-complete.
\end{theorem}

\begin{proof}
\end{proof}

 
%\subsection{Two-way transducers}\label{sec-2way}
%
%\zhilin{moved two-way automata and transducers from Section 2 here} 
% 
%\begin{definition}[Two-way finite-state automata] \label{def:2nfa}
%	A \emph{(nondeterministic) two-way finite-state automaton}
%	(\FFA{}) over a finite alphabet $\ialphabet$ is a tuple $\Aut =
%	(\ialphabet, \EndLeft, \EndRight, \controls, q_0, \finals, \transrel)$ where 
%	$\controls$ is a finite set of 
%	states, $\EndLeft$ (resp.~$\EndRight$) a left (resp.~right) input tape end 
%	marker, $q_0\in \controls$ is
%	the initial state, $\finals\subseteq \controls$ is a set of final states, and 
%	$\transrel$ is the
%	transition relation  $\transrel\subseteq \controls \times 
%	\overline{\ialphabet}\times \{\Left, \Stay, \Right\}\times \controls$. 
%	%with $\overline{\ialphabet} := \ialphabet \cup \{\EndLeft,\EndRight\}$.
%	Here, we assume %$\EndLeft, \EndRight \notin \ialphabet$, and 
%	that
%	there are no transitions that take the head of the tape past the left/right
%	end marker (i.e.~$(p,\EndLeft,\Left,q), (p,\EndRight,\Right,q) \notin
%	\transrel$ for every $p, q \in \controls$).
%	%\tl{not sure you want to use $\leftarrow, \rightarrow$?}
%	%    \anthony{Just defined macros. Please use generic macros in the definitions
%	%    guys.}
%	
%	A \emph{(nondeterministic one-way) finite-state automaton} (\FA{})
%	is a \FFA{} such that $\transrel \subseteq \controls \times \overline{\ialphabet} \times
%	\{\Right,\Stay\} \times \controls $.
%	%    
%	%A two-way \emph{sweeping automaton} (\SFFA{})  is a \FFA{} performing head reversal only when the input head is visiting the endmarkers. 
%
%	Whenever understood we will only tacitly mention $\ialphabet$, 
%	$\EndLeft$, and $\EndRight$ in $\Aut$.  
%\end{definition}
%
%The notion of runs of \FFA{} on an input string is exactly the same as that of
%Turing machines on a read-only input tape. More precisely, for a string 
%$w = a_1 \dots a_n$, a \emph{run} of $\Aut$ on $w$
%%(with $a_0 = \EndLeft$ and $a_{n+1} = \EndRight$)
%is a sequence of pairs $(q_0,i_0),\ldots, (q_m,i_m) \in \controls \times [0, n+1]$ 
%defined as follows. Let $a_0 = \EndLeft$ and $a_{n+1} = \EndRight$. The
%following conditions then have to be satisfied: $i_0 = 0$, and for every $j \in [0, m-1]$, we have $(q_j,a_{i_j}, dir, q_{j+1}) \in
%\transrel$ and $i_{j+1} = i_j + dir$ for some $dir \in  \{\Left, \Stay, \Right\}$.
%
%%\begin{itemize}
%%    \item $i_0 = 0$, and
%%    \item for every $j \in [m-1]$, we have $(q_j,a_{i_j}, dir, q_{j+1}) \in
%%        \transrel$ and $i_{j+1} = i_j + dir$ for some $dir \in  \{\Left, \Stay, \Right\}$.
%%\end{itemize}
%The run is said to be \defn{accepting} if $i_m = n+1$ and $q_m \in \finals$.
%A string $w$ is \defn{accepted} by $\Aut$ if there is an accepting run of
%$\Aut$ on $w$. The set of strings accepted by $\Aut$ is denoted by $\Lang(\Aut)$,
%a.k.a., the language \defn{recognised} by $\Aut$.
%%Since we deal with computational complexity in the sequel, we define
%The \defn{size} $|\Aut|$ of $\Aut$ is defined to be $|\controls|$; this will
%be needed when we talk about computational complexity.
%
%
%
%
%In the rest of this paper, %\FA{}s refer to $\varepsilon$-free \FA{}s where directions in transitions are omitted. Moreover, 
%for simplicity of notations we omit the two end markers $\EndLeft, \EndRight$ in \FA{}s and assume that $\transrel \subseteq \controls \times \ialphabet \times    \{\Right,\Stay\} \times \controls$. 
%%
%For convenience, we will also refer to an \FA{} without initial and final states, that is, a pair $(Q, \delta)$, as a \emph{transition graph}.
%
%%====================================================================
%%A \emph{nondeterministic finite automaton} (NFA) $\cA$ on $\Sigma$ is a tuple $(Q, \delta, q_0, F)$, where $Q$ is a finite set of \emph{states}, $q_0 \in Q$ is the \emph{initial} state, $F \subseteq Q$ is the set of \emph{final} states, and $\delta \subseteq Q \times \Sigma \times Q$ is the \emph{transition relation}. For a string $w = a_1 \dots a_n$, a \emph{run} of $\cA$ on $w$ is a state sequence $q_0 \dots q_n$ such that for each $i \in [n]$, $(q_{i-1}, a_i, q_i) \in \delta$. A run $q_0 \dots q_n$ is \emph{accepting} if $q_n \in F$. A string $w$ is \emph{accepted} by $\cA$ if there is an accepting run of $\cA$ on $w$. We use $\Ll(\cA)$ to denote the language defined by $\cA$, that is, the set of strings accepted by $\cA$. We will use $\cA, \cB, \cdots$ to denote NFAs. 
%%%An NFA $\cA$ is \emph{deterministic} if for each $(q, \sigma) \in Q \times \Sigma$, there is at most one $q' \in Q$ such that $(q, a, q') \in \delta$. An NFA $\cA$ is \emph{complete} if for each $(q, \sigma) \in Q \times \Sigma$, there is at least one $q' \in Q$ such that $(q, a, q') \in \delta$. We assume that all NFA considered in this paper are complete.  An NFA $\cA$ is \emph{unambiguous} if for each word $w$, there is \emph{at most one accepting} run of $\cA$ on $w$.
%%For a string $w= a_1 \dots a_n$, we also use the notation $q_1 \xrightarrow[\cA]{w} q_{n+1}$ to denote the fact that there are $q_2,\dots, q_n \in Q$ such that for each $i \in [n]$, $(q_i, a_i, q_{i+1}) \in \delta$.  For an NFA $\cA=(Q, \delta, q_0, F)$ and $q, q' \in Q$, we use $\cA(q,q')$ to denote the NFA obtained from $\cA$ by changing the initial state to $q$ and the set of final states to $\{q'\}$. The \emph{size} of an NFA $\cA=(Q, \delta, q_0, F)$, denoted by $|\cA|$, is defined as $|Q|$, the number of states. For convenience, we will also call an NFA without initial and final states, that is, a pair $(Q, \delta)$, as a \emph{transition graph}. 
%%=========================================================
%
%
%
%%The following result is standard and can be found in textbooks on automata theory
%%
%%\begin{proposition}\label{prop-2nfa-nfa}
%%	Every \FFA{} $\Aut$ can be transformed in exponential time into an equivalent \FA{} of size $2^{\bigO(|\Aut| \log |\Aut|)}$. 
%%	%	Moreover, the equivalent
%%	%    NFA can be computed in exponential time. 
%%	Moreover, every \FA{} can be transformed in polynomial time into an $\varepsilon$-free \FA{}, that is, an \FA{} where $\transrel\subseteq \controls \times \overline{\ialphabet} \times   \{\Right\} \times \controls $.
%%\end{proposition}
%% 
%%
%%For latter reference, here we briefly mention the construction of \FA{}s from \FFA{}s in \cite{HU79}: For each  \FFA{} $\Aut=(\controls, q_0, \finals, \transrel)$, each state of the equivalent \FA{} is a vector of states from $\controls$ of \emph{odd} length, say $(q_1, \ldots, q_{2n+1})$, such that all the states of even (resp. odd) indices are mutually distinct.
%
% 
%
%\smallskip
%\noindent\textbf{Operations of \FA{}s.} For an FA $\Aut=(Q, q_0, F, \delta)$, $q \in Q$ and $P \subseteq Q$, we use $\Aut(q, P)$ to denote the FA $(Q, q, P, \delta)$, that is, the FA obtained from $\Aut$ by changing the initial state and the set of final states to $q$ and $P$ respectively. We use $q \xrightarrow[\Aut]{w} q'$ to denote the fact that a string $w$ is accepted by $\Aut(q, \{q'\})$. 
%
%
%Given two \FA{}s $\Aut_1 = (Q_1, q_{0,1}, F_{1}, \delta_1)$ and $\Aut_2 = (Q_2, q_{0,2}, F_2, \delta_2)$, the \emph{product} of $\Aut_1$ and $\Aut_2$, denoted by $\Aut_1 \times \Aut_2$, is defined as $(Q_1 \times Q_2, (q_{0,1}, q_{0,2}), F_1 \times F_2, \delta_1 \times \delta_2)$, where $\delta_1 \times \delta_2$ is the set of tuples $((q_1,q_2), a, (q'_1, q'_2))$ such that $(q_1, a, q'_1) \in \delta_1$ and $(q_2, a, q'_2) \in \delta_2$. Evidently, we have $\Lang(\Aut_1 \times \Aut_2) = \Lang(\Aut_1) \cap \Lang(\Aut_2)$.
%
%We note that \FFA{} and \FA{}recognise precisely the same class of languages, i.e., 
%\emph{regular languages}, and thus are expressively equivalent to regular expressions \cite{HU79}. 
%%It is well-known (e.g. see \cite{HU79}) that regular expressions and \FA{} are 
%%expressively equivalent, and generate precisely all \emph{regular languages}.
%In particular, from a regular expression, an equivalent \FA{} can be constructed 
%in linear time. Moreover, regular languages are closed under Boolean
%operations, i.e., union, intersection, and complementation.
%%In particular, given two \FA{} $\cA_1=(Q_1, \delta_1, q_{0,1}, F_1)$ and
%%$\cA_2=(Q_2, \delta_2, q_{0,2}, F_2)$ on $\Sigma$, the intersection $\Ll(\cA_1)
%%\cap \Ll(\cA_2)$ is recognised by the \emph{product automaton} $\cA_1 \times
%%\cA_2$ of $\cA_1$ and $\cA_2$ defined as $(Q_1 \times Q_2, \delta, (q_{0,1}, q_{0,2}), F_1 \times F_2)$, where $\delta$ comprises the transitions $((q_1, q_2), a, (q'_1, q'_2))$ such that $(q_1, a, q'_1) \in \delta_1$ and $(q_2, a, q'_2) \in \delta_2$.  
%
% 
%%We will start by giving the precise definition of two-way and one-way  finite transducers. 
%%which %are respectively two-way and one-way finite-state automata extended with outputs.  
%\begin{definition}[Finite-State Transducers]
%	Let $\ialphabet$ be an alphabet. A \emph{nondeterministic two-way finite  transducer} (\FFT{}) $\Transducer$  over $\ialphabet$ is a tuple $(\ialphabet, \EndLeft, \EndRight, \controls, q_0, \finals, \transrel)$, where $\transrel$ is  a finite subset of $\controls \times \overline{\ialphabet}\times \{\Left, \Stay, \Right\}\times 
%	\controls \times \ialphabet^*$, satisfying the syntactical constraints of \FFA{}s, and the additional constraint that the output must be $\epsilon$ when reading $\EndLeft$ or $\EndRight$. Formally, for each transition $(q, \EndLeft, dir, q', w)$ or $(q, \EndRight, dir, q', w)$ in $\delta$, we have $w=\epsilon$.
%	%
%	%    A \emph{nondeterministic two-way (finite) \emph{transducer}} (\FFT{}) over 
%	%    $\ialphabet$ is a tuple $\Transducer = (\ialphabet, \EndLeft, \EndRight, \controls, q_0, \finals, \transrel)$ where  $\controls$, $\EndLeft$, $\EndRight$, $q_0$, and $\finals$ are precisely the same as those of Definition~\ref{def:2nfa}
%	%
%	%and 
%	%    $\transrel$ is the
%	%transition relation  $\transrel\subseteq \controls \times 
%	%    \overline{\ialphabet}\times \{\Left, \Stay, \Right\}\times 
%	%    \controls \times \ialphabet_\epsilon$ with
%	%    $\overline{\ialphabet} := \ialphabet \cup \{\EndLeft,\EndRight\}$.
%	%    Here, we assume $\EndLeft, \EndRight \notin \ialphabet$, and that
%	%    there are no transitions that take the head of the tape past the left/right
%	%    end marker. 
%	%
%	A (nondeterministic one-way) finite transducer (\FT{}) over
%	$\ialphabet$ is a \FFT{} such that $\transrel \subseteq \controls \times \overline{\ialphabet} \times
%	\{\Right,\Stay\} \times \controls \times \ialphabet^*$.
%	%A sweeping \FFT{} (\SFFT{}) is defined similarly to \SFFA.
%	%    whose transition relation contains only tuples of the form
%	%    $(p,a,dir,q,b)$, where $dir \in \{\Stay,\Right\}$.
%\end{definition}
%%\zhilin{I simplified the above definition slightly, please check. I also extend the 2FTs to allow multiple output symbols in one transition. Moreover, I assume that for each transition $(q, \EndLeft, \Right/\Stay, q', b)$, we have $b=\epsilon$. Similarly for $\EndRight$.} \tl{polish slightly, hopefully ok.}
%%
%%\anthony{Define the semantics of \FFT{} as function $f: \ialphabet^* \to
%%\ialphabet^*$}.\zhilin{Semantics defined below. Please check.}
%%
%The notion of runs of \FFT{}s on an input string can be seen as a generalisation 
%of \FFA{}s by adding outputs. More precisely, given a string $w = a_1 \dots a_n$, a \emph{run} of $\Transducer$ on $w$
%%(with $a_0 = \EndLeft$ and $a_{n+1} = \EndRight$)
%is a sequence of tuples $(q_0, i_0, w'_0),\ldots, (q_m, i_m, w'_m) \in \controls \times
%[0, n+1] \times \Sigma^*$ 
%such that, if $a_0 =\ \EndLeft$ and $a_{n+1} =\ \EndRight$, 
%we have $i_0 = 0$, and  for every $j \in [0, m-1]$, $(q_j, a_{i_j}, dir, q_{j+1}, w'_j) \in
%\transrel$, $i_{j+1} = i_j + dir$ for some $dir \in \{\Left, \Stay, \Right\}$, and $w'_0 = w'_m = \varepsilon$.
%The run is said to be \defn{accepting} if $i_m = n+1$ and $q_m \in \finals$.
%When a run is accepting, $w'_0 \cdots w'_m$ is said to be the \emph{output} of the
%run. Note that some of these $w'_i$'s could be empty strings.
%A word $w'$ is said to be an output of $\Transducer$ on $w$ if there is an accepting run of
%$\Transducer$ on $w$ with output $w'$. We use $\Tran(\Transducer)$ to denote the
%\emph{transduction} defined by $\Transducer$, that is, the relation comprising
%the pairs $(w,w')$ such that $w'$ is an output of $\Transducer$ on $w$. 
%
%We remark that a \FFT{} usually defines a relation. We shall speak of \emph{functional
%	transducers}, i.e., transducers that define functions instead of relations. (For instance, deterministic transducers are always functional.) 
%%In this paper, transducers 
%%define functions, but can be non-deterministic.
%
%To take into consideration the outputs of transitions, we define the \emph{size} $|\Transducer|$ of $\Transducer$ as the sum of the sizes of transitions in $\Transducer$, where the size of a transition $(q, a, dir, q', w')$ is defined as $|w'|+1$. With the assumption that only $\epsilon$ can be outputted when reading $\EndLeft$ or $\EndRight$, for simplicity, we omit the two end markers $\EndLeft$ and $\EndRight$ in \FT{}s, that is, $\transrel \subseteq \controls \times \ialphabet \times \{\Right,\Stay\} \times \controls \times \ialphabet^*$. Note that each accepting run of an \FT{} has to read through the input string and stop in the right end.
%
%
%
%
%
%\begin{example}\label{exmp-ft}
%	We give two examples of \FFT{}s: %(1) erasing \texttt{a} from  a string, (2) 
%	(1) the function \textbf{escapeString}, and (2) the  function \textbf{reverse}.
%	
%	The first function backslash-escapes every occurrence of \texttt{'} and 
%	\texttt{"}. This can be modelled by an \FT{} with a single state $q_0$,
%	transitions 
%	%$(q_0, \EndLeft, 1, q_1,\epsilon)$,
%	$(q_0, \ell, 1, q_0, \ell)$ for each $\ell \neq  \texttt{'}$  or $\texttt{"} $, 
%	$(q_0,\texttt{'}, 1, q_0, \textbackslash\texttt{'})$, 
%	$(q_0,\texttt{"}, 1, q_0, \textbackslash\texttt{"})$,  
%	%and
%	%$(q_1,\EndRight,0,q_2,\epsilon)$. 
%	and the final state $q_0$.
%	%\zhilin{I removed the two end markers.}
%	%
%	%    The second transducer backslash-escapes every occurrence of \texttt{'} and 
%	%    \texttt{"}. This can also be done by a \FT{} in a similar way. Instead of
%	%    providing the formal definition, we depict this informally as a 
%	%    state-diagram in Figure
%	%    \ref{fig:escapeString}, bearing in mind that 
%	%    %the transitions for the left/right end markers are omitted, and that
%	%     the transition label
%	%    $a/w$ means \emph{read $a$, and meanwhile output $w$}.
%	%%$a/w$ denotes 
%	%
%	The second function requires us to use a \FFT{}, which we will only describe
%	informally. The transducer $\Transducer_{\mathsf{reverse}}$ will firstly move to $\EndRight$ of the input tape
%	without outputting any symbol. It then scans the input from
%	right to left, while outputting the symbol that is read.
%	When $\EndLeft$ is reached, it moves its input head right to $\EndRight$ (without outputting any further symbol), and accepts.     \qed
%\end{example}
%
%
%
%
%%Let $\Transducer$ be a 2NPT with $k$ parameters $y_1,\cdots, y_k$ and $\Aut$ be an NFA. Then the \emph{preimage} of $\Aut$ w.r.t. $\Transducer$, denoted by $\Pre_\Transducer(\Aut)$, is the set of tuples $(w, w_1,\cdots, w_k)$ such that there is an accepting run of $\Transducer$ on $w$ producing an output $w' \in \Lang(\Aut)$, equipped with the parameters $w_1,\cdots, w_k$.
%
%
%\begin{lemma}\label{lem-2pt}
%	The  regularity condition  \prerec{} holds for string functions definable in \FFT{}s, with $\ell(|\Transducer|, |\Aut|) = 2^{\bigO(|\Transducer||\Aut|\log (|\Transducer||\Aut|))}$. %, where $T$ is a  \PPT{}, and $\Aut$ is a conjunctive  \FFA{}. 
%	%Let $\Transducer$ be a \PPT{} and $\Aut$ be a conjunctive \FA{} $\Aut$. Then $\Pre_\Transducer(\Aut)$ is a recognisable relation. Moreover, a representation of $\Pre_\Transducer(\Aut)$, whose atom size is bounded by $2^{O(|\Transducer||\Aut|\log (|\Transducer||\Aut|))}$, can be computed effectively. Moreover, each disjunct of the representation can be nondeterministically computed in $2^{O(|\Transducer||\Aut|\log (|\Transducer||\Aut|))}$ space.
%\end{lemma}
%
%\tl{to adapt this to 2FTs, as 2PTs are not needed.}
%\begin{proof}
%	Assume a \PPT{} $\Transducer=(X, Q, q_0, F, \delta)$ with $X = \{x_1,\cdots, x_\arity\}$ and a conjunctive \FA{} $\Aut = ((Q', \delta'), \conacc')$ with $\conacc' \subseteq Q' \times Q'$. %We first introduce some notations. 
%	Let $\oalphabet = \ialphabet \cup X$.
%	
%	To compute $\Pre_\Transducer(\Aut)$, we construct a conjunctive \FFA{} %\footnote{Conjunctive \FFA{}s are defined similarly to conjunctive \FA{}s.} 
%	$\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q}$, %defined as follows. 
%	%and $\Aut[S]$ defined below.
%	%
%	where  $q \in F$ and  $\conacc_{x_1}, \cdots, \conacc_{x_\arity} \subseteq Q' \times Q'$.   
%	%The conjunctive \FFA{} $\cB_{\Transducer, \Aut, S_{x_1}, \cdots, S_{x_k}, q}$ is constructed 
%	Intuitively this is done from $\Transducer$  by checking for an accepting run of $T$ on $w$ ending at state $q$, and simulating an accepting run of $\Aut$ on the output of $\Transducer$. States of $\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q}$ comprise $(q,q') \in Q \times Q'$. 
%	%In particular, 
%	When a transition of $\Transducer$ outputs a string $w'$ from $\oalphabet^*$ where some parameter $x_i$ appears (instead of a constant string), for each occurrence of $x_i$ in $w'$, a pair of states $(q_1', q_2')$ is nondeterministically selected from $\conacc_{x_i}$, and the second component of the state of $\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q}$ will be updated from $q_1'$ to $q_2'$ to mimic a possible instantiation of $x_i$.  
%	%\tl{zhilin, I am not quite clear about the para, $y_1$ is a typo of $x_1$? I wrote a para above; please check}
%	%(instead of materialising the output), where $S_{x_1}$ is used to jump over $y_1$ when $x_1$ is the output of a transition of $\Transducer$, similarly for $S_{x_2}, \cdots, S_{x_k}$. 
%	More precisely, $\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q}$ is defined as
%	%\begin{enumerate} 
%	%\item 
%	%the conjunctive \FFA{} 
%	$\Aut'' = ((\controls'', \transrel''), \conacc'')$, where $Q'' = Q \times Q'$, $\conacc'' = \{((q_0, p), (q, p')) \mid (p, p') \in \conacc'\}$, and the transition relation $\transrel''$ comprises the tuples $((q_1, q'_1), a, dir, (q_2, q'_2))$ such that there is $w' \in \oalphabet^*$ satisfying that $(q_1, a, dir, q_2, w') \in \transrel$, and either
%	\begin{itemize}
%		\item $w' \in \ialphabet^*$  and $q'_1 \xrightarrow[\Aut]{w'} q'_2$, or
%		%
%		\item suppose $w' = w'_1 x_{i_1} \ldots w'_{s} x_{i_{s}} w'_{s+1}$ for some $s \ge 1$, $w'_j \in \ialphabet^*$ for each $j \in [s+1]$,  and $i_j \in [\arity]$ for each $j \in [s]$, then there are states $p_0, p_1, \ldots, p_{2s+1} \in \controls'$ satisfying that $p_0 = q'_1$, $p_{2s+1} = q'_2$, and 
%		$$p_0 \xrightarrow[\Aut]{w'_1} p_1 \xrightarrow{\conacc_{x_{i_1}}} p_2\ \ldots\ p_{2s-2} \xrightarrow[\Aut]{w'_s}p_{2s-1} \xrightarrow{\conacc_{x_{i_s}}} p_{2s} \xrightarrow[\Aut]{w'_{s+1}} p_{2s+1},$$ 
%		where $p_{2j-1} \xrightarrow{\conacc_{x_{i_j}}} p_{2j}$ means $(p_{2j-1}, p_{2j}) \in \conacc_{x_{i_j}}$ for each $j \in [s]$.
%	\end{itemize}
%	%
%	%
%	%\item Define $\cB_{\Transducer, \Aut, S_{x_1}, \cdots, S_{x_k}, q}$ as $((Q''', \delta'''), S')$, where $S' = \{(\vec{\rho}_1, \vec{\rho}_2) \mid  (q'_1,q'_2) \in S, \vec{\rho}_1[1] =(q_0,q'_1), \vec{\rho}_2[|\vec{\rho}_2|] = (q, q'_2) \}$.
%	%\end{enumerate} 
%	It is easy to see that  the size of $\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q}$ is at most $|\Transducer||\Aut|$ and $|\conacc''| = |\conacc'|$.   
%	%$2^{O(|T||\Aut| \log(|T||\Aut|))}$.   
%	
%	%For $S \subseteq Q' \times Q'$, let $\Aut[S]$ denote the product of $\Aut(q'_1, \{q'_2\})$ for $(q'_1,q'_2) \in S$ (cf. Section~\ref{sec:prelim}, {Operations of NFAs.}). Since $S$ contains at most $|Q'|^2=|\Aut|^2$ many elements, the size of $\Aut[S]$ is bounded by $|\Aut|^{|\Aut|^2} \approx 2^{O(|\Aut|^2 \log |\Aut|)}$.
%	\smallskip
%	\noindent
%	\emph{Claim.} %For each tuple of strings $(w, w_1,\cdots, w_k)$, 
%	$(w, w_1,\cdots, w_\arity) \in \Pre_\Transducer(\Aut)$ iff there are $\conacc_{x_1}, \cdots, \conacc_{x_\arity} \subseteq Q' \times Q'$ and $q \in F$ such that $w \in \Lang(\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q})$ and $w_i \in \Lang(\Aut[\conacc_{x_i}])$ for each $i \in [r]$, where $\Aut[\conacc_{x_i}]=((Q', \delta'), \conacc_{x_i})$. [The proof of the claim is given in Appendix~\ref{appendix:sec-2way}; it crucially relies on that $T$ is functional otherwise it would \emph{not} be correct.]
%	\smallskip
%	
%	Thus, $\Pre_\Transducer(\Aut)$ is a recognisable relation equal to
%	\[
%	\bigcup_{\conacc_{x_1}, \cdots, \conacc_{x_\arity} \subseteq Q' \times Q', q\in F} \Lang(\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity},q}) \times \Lang(\Aut[\conacc_{x_1}]) \times \cdots  \times \Lang(\Aut[\conacc_{x_\arity}]).\]
%	%
%	
%	To represent $\Pre_\Transducer(\Aut)$, we transform the conjunctive \FFA{} $\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity},q}$ to a union of conjunctive \FA{}s as follows: Transform $\Aut''$ into a one-way transition graph $(\controls''',\delta''')$, where $\controls'''$ are vectors of states of $\Aut''$ of lengths at most $2|\controls''|-1$ (cf. Proposition~\ref{prop-2nfa-nfa}). Then $\Lang(\cB_{\Transducer, \conacc_{x_1}, \cdots, \conacc_{x_\arity},q})$ is the union of $\Lang(((\controls''',\delta'''), \conacc''))$ for $\conacc'' \subseteq \controls''' \times \controls''',$ which comprises nondeterministically selected pairs $(\vec{\rho}_1, \vec{\rho}_2) \in \controls''' \times \controls'''$, one for each $(p, p') \in \conacc'$, such that $\vec{\rho}_1[1] =(q_0, p)$ and  $\vec{\rho}_2[|\vec{\rho}_2|] = (q, p')$.
%	%that is computed nondeterministically from $\cB_{\Transducer, S_{x_1}, \cdots, S_{x_k},q}$ and $S'$ as follows:  For each $(p, p') \in S$, nondeterministically select one pair $(\vec{\rho}_1, \vec{\rho}_2) \in \controls''' \times \controls'''$ satisfying $\vec{\rho}_1[1] =(q_0, p)$ and  $\vec{\rho}_2[|\vec{\rho}_2|] = (q, p')$, then put it into $S''$.
%	
%	Since the size of each conjunctive \FA{} $((\controls''',\delta'''), \conacc'')$ is $ 2^{\bigO(|\Transducer||\Aut|\log (|\Transducer||\Aut|))}$, we conclude that 
%	the \prerec{} assumption holds for string functions definable in \PPT{}s with $\ell(|\Transducer|, |\Aut|) = 2^{O(|\Transducer||\Aut|\log (|\Transducer||\Aut|))}$.
%	%$\Pre_\Transducer(\Aut)$ is a recognisable relation and a representation of $\Pre_\Transducer(\Aut)$, whose atom size is bounded by $2^{O(|\Transducer||\Aut|\log (|\Transducer||\Aut|))}$, can be constructed effectively.
%\end{proof}
%
%Lemma~\ref{lem-2pt} and Theorem~\ref{thm-generic-dec} entail %by some simple calculation, we deduce that 
%%given a string manipulating program $S$ in SSA form where string functions are modelled by \PPT{}s, 
%one can decide the path feasibility of a symbolic execution $S$ with \PPT{}s in 
%%nondeterministic 
%%$$O((\rcdim(\varphi)+2)^{\rcdep(\varphi)} (f^{\langle \rcdep(\varphi) \rangle}(|\varphi|, |\psi|))^2 \log f^{\langle \rcdep(\varphi) \rangle}(|\varphi|, |\psi|))$$ 
%%space, where $f(j, k) = 2^{jk \log (j k)}$. 
%nondeterministic 
%
%\smallskip
%\hspace{1cm} $\tower(\rcdep(S), \bigO(\rcphi(S) \rcpsi(S)  \log(\rcphi(S) \rcpsi(S)))$ 
%\smallskip
%
%\noindent space (which can be even made in \emph{deterministic} space by Savitch's theorem \cite{Savitch70}). Here $\tower(1, k)= 2^k$ and $\tower(j+1, k) = 2^{\tower(j, k)}$. 
%After the result we sketch the lower bound.
%%We conclude that the path feasibility of such string manipulating programs  can be decided in $\rcdep(S)$-exponential space.
%%Moreover, we have a matching lower bound whose proof is sketched below.
%%
%\begin{theorem} \label{thm:two-way}
%	Given a symbolic execution $S$ with \PPT{}s, the path feasibility of $S$ can be decided in $\rcdep(S)$-exponential space. 
%	%Moreover,  for any $\expheight$, checking path feasibility is $\expheight$-$\expspace$-hard.
%\end{theorem}
%======================================================================

%\tl{will see later where to put this stuff}
%\subsubsection{Reversal-bounded case}
%
%In practice, many string functions need only a small number of reversals for the reading head, rather than full two-way transducers. 
%E.g., the reading head for one-way \PT{} (resp. the string reverse function) needs $0$ (resp. $2$) reversal(s).
%
%Let $k \in \Nat$. A $k$-reversal bounded \PPT{} $\Transducer$ ($k$-\RBPPT{}) is such that in every run of $\Transducer$, the reading direction is reversed at most $k$ times. 
%Notice that $k$ must be even since accepting runs must stop on the right end of input strings. 
%Evidently, $0$-reversal bounded \PPT{}s are precisely one-way \PT{}s.   
%
%
%%Therefore, we have: 
%%
%\begin{lemma}\label{lem-rb2pt}
%	The regularity condition \prerec{} holds for string functions definable in $k$-\RBPPT{}s, with $\ell(|\Transducer|, |\Aut|) = (|\Transducer||\Aut|)^{k+1}$.
%\end{lemma}
%
%We follow the construction in the proof of Lemma~\ref{lem-2pt}. One can see that the size of \FFA{} $\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q}$  is bounded by $|\Transducer| |\Aut|$. Moreover, as $T$ is $k$-reversal bounded, so is $\cB_{\Transducer, \Aut, \conacc_{x_1}, \cdots, \conacc_{x_\arity}, q}$. Therefore, according to the construction of \FA{} from \FFA{}  (cf. \cite{HU79}), we have that the size of each obtained conjunctive \FA{} in the recognisable relation (cf. the proof of Lemma~\ref{lem-2pt}) is at most $ (|\Transducer||\Aut|)^{k+1}$. 
%
%Combing Theorem~\ref{thm-generic-dec} and Lemma~\ref{lem-rb2pt}, we have:
%
%\begin{theorem} \label{thm-rb-2pt}
%	Let  $k \in \Nat$. The path feasibility of string constraints with $k$-\RBPPT{}s is in 2-$\expspace$. 
%\end{theorem}
%%
%To see Theorem~\ref{thm-rb-2pt}, we invoke Theorem~\ref{thm-generic-dec} again. One can observe that the space required by the instantiation of the generic procedure is 
%
%\smallskip
%\hspace{1.5cm} $\mathcal{O}(\rcphi(S)^{(k+1)+(k+1)^2+...+(k+1)^m}\cdot  \rcpsi(S)^{(k+1)^m})$
%\smallskip
%
%\noindent (where $m=\rcdep(S)$), which is doubly exponential in the size of $S$. 
%




%Crucially, symbolic executions where string functions are given by $k$-\RBPPT{}s can be translated to those where string functions are given by only \PT{}s and a special transducer $\Transducer_{\sf reverse}$ for the string reverse function  (cf. Example~\ref{exmp-ft} in Section~\ref{sec:framework}).  
%%%==========================================
\hide{
	\begin{proposition} \label{prop:trans}
		Any symbolic execution $S$ where string functions are given by $k$-\RBPPT{}s can be translated to $S'$ where string functions are given by \PT{}s and $\Transducer_{\sf reverse}$, and $ \rcdep(S')\in \mathcal{O}(k\cdot \rcdep(S))$. 
	\end{proposition}
}
%%%==========================================

%\hide{
%Crucially, symbolic executions where string functions are given by \SPPT{}s can be translated in polynomial time to those where string functions are given by only \PT{}s and a special transducer $\Transducer_{\sf reverse}$ for the string reverse function  (cf. Example~\ref{exmp-ft} in Section~\ref{sec:framework}).  
%
%
%\begin{proposition}\label{prop-sweep-rb}
%Suppose $\Transducer=(\controls, X, q_0, \finals, \transrel)$ is a \emph{functional} \SPPT{}  with $X= \{x_1,\ldots, x_\arity\}$. Then for each $(w, w', w_1,\ldots, w_\arity) \in \transet(\Transducer)$, there is an accepting run of $\Transducer$ on $w$, equipped with $w_1,\ldots, w_\arity$, with the output $w'$, such that the run contains at most $2(|\controls|-1)$ reversals.
%\end{proposition}
%
%From Proposition~\ref{prop-sweep-rb}, we deduce the following result.
%
%\begin{proposition} \label{prop:trans}
%	Any symbolic execution $S$ where string functions are given by \SPPT{}s can be translated to $S'$ where string functions are given by \PT{}s and $\Transducer_{\sf reverse}$, and $ \rcdep(S')\in \mathcal{O}(\rcphi(S) \cdot \rcdep(S))$. 
%\end{proposition}
%
%Proposition~\ref{prop:trans} is shown in
%\shortlong{the full version}{Appendix~\ref{app-rb-2pt}}.
%Intuitively, a run of a \SPPT{} $\Transducer$ can be split into $2(n-1)$ subruns (where $n$ is the number of states of $\Transducer$), each travelling in a single direction.
%We simulate the subruns with $2(n-1)$ one-way \PT{}s whose outputs are concatenated.
%Right-to-left subruns are simulated left-to-right, and thus the output must be reversed before concatenation.
%}


%Proposition~\ref{prop:trans} is shown in
%\shortlong{the full version}{Appendix~\ref{app-rb-2pt}}.
%Intuitively, a run of a $k$-\RBPPT{} can be split into $k$ runs, each travelling in a single direction.
%We simulate the runs with $k$ one-way \PT{}s whose outputs are concatenated.
%Right-to-left runs are simulated left-to-right, and thus the output must be reversed before concatenation.

\OMIT{
We are also interested in the question whether one could obtain lower complexity bounds for more specific string functions. In particular, we will examine \PT{}s, 
%$\Transducer_{\sf reverse}$ (cf. Example~\ref{example:2pt}) and  $\Transducer_{\sf replaceall}$
reverse function modelled by $\Transducer_{\mathsf{reverse}}$ (cf.\ Example~\ref{exmp-ft}), concatenation and replaceall function modelled by $\Transducer_{\mathsf{concat}}$ and $\Transducer_{\replaceall_p}$ respectively (cf.\ Example~\ref{example:2pt}). To instantiate the generic decision procedure for these functions, we verify the regularity condition \prerec{} for them as follows.
%The  \prerec{} assumption for \PT{}s and $\Transducer_{\sf reverse}$. Indeed,
One may notice that although $\Transducer_{\mathsf{reverse}}$ is a two-way transducer, its pre-image does \emph{not} bring an exponential blowup as general \PPT{}s would have. 

\begin{lemma}\label{lem-1pt}
	The regularity condition \prerec{} holds for string functions definable in \PT{}s or $\Transducer_{\mathsf{reverse}}$, with $\ell(|\Transducer|, |\Aut|) = |\Transducer||\Aut|$.
\end{lemma}

The proof is the same as Lemma~\ref{lem-2pt} except constructing $\cB_{\Transducer, \Aut, \conacc_{x_1}, \ldots, \conacc_{x_\arity}, q}$ is simpler, with size at most $|\Transducer| |\Aut|$, since the transformation from  conjunctive \FFA{} to conjunctive \FA{} is not needed. For $\Transducer_{\sf reverse}$, the pre-image is given by reversing the direction of each transition of $\Aut$ and swapping initial and final states. 

Furthermore, Proposition~\ref{prop-replace-pt} entails that  $\Transducer_{\replaceall_p}$ is of size $2^{\mathcal{O}(|p|^c)}$ for some constant $c > 0$. It follows from Theorem~\ref{thm-generic-dec} and Lemma~\ref{lem-1pt} that we have: 

\begin{theorem}\label{cor-s2pt}
	The path feasibility of string constraints with \PT{}s, replaceall, and reverse is $\expspace$-complete.
\end{theorem}
%
%\begin{theorem} \label{thm-s2pt}
%The path feasibility of string constraints with \SPPT{}s is $\expspace$-complete. 
%\end{theorem}

We remark the above logic also includes concatenation.
The lower bound is from the $\expspace$-hardness of path feasibility of straight-line string constraints with concatenation and one-way (non-parametric) transducers,  both of which are special cases of \PT{}s~\cite{LB16}.
}
%
%\subsection{Length constraints}

==> related.tex <==
%!TEX root = main.tex



 

\section{Related work}\label{sec-rel}

\tl{This is largely copied from popl18. to be adapted}

We now discuss some related work. We split our discussion into two categories: (1) theoretical results in terms of decidability and complexity; (2) practical (but generally incomplete) approaches used in string solvers.  

%We emphasise work on $\replaceall$ functions as they are our focus. 

\paragraph{Theoretical Results}
%We have discussed in Section \ref{sec:intro} works on string constraints with 

The theory of strings with concatenation. This research programme builds on
the question of solving satisfiability of \emph{word equations}, i.e., a
string equation $\alpha = \beta$ containing concatenation of string constants
and variables. Makanin showed decidability \cite{Makanin}, whose upper bound
was improved to PSPACE in \cite{P04} using a word compression technique. 
A simpler algorithm was in recent years proposed in \cite{J17} using
the recompression technique. The best lower bound for this problem is still NP,
and closing this complexity gap is a long-standing open problem. Decidability
(in fact, the PSPACE upper bound) can be retained in the presence of regular
constraints (e.g. see \cite{Schulz}). This can be extended to existential theory
of concatenation with regular constraints using the technique of \cite{buchi}.

%The replace-all operator cannot be expressed by the concatenation operator alone. For 
%this reason, our decidability of the fragment of $\strline[\replaceall]$ cannot
%be derived from the results from the theory of concatenation alone.

%Our work is closely related to solving word equations, which are a conjunction of equations of $v=w$, where $v, w$ are concatenation of string constants and variables. The computational complexity of this problem remains unknown, with the best lower and upper bounds being NP and PSPACE respectively. Makanin %refuted a conjecture 
%showed, perhaps surprisingly, that the problem is decidable \cite{Makanin}, and %Plandowski's  on the decidability and complexity of satisfiability for word equations, i.e., 
%Plandowski explored an approach of compression and proposed a PSPACE algorithm \cite{P04}.  This is the best bound up to date, though a simpler PSPACE algorithm with smaller space requirement (nondeterministic $O(n \log n)$ space) was proposed by Jez \cite{J16}, based on compression. Very recently, Jez \cite{J17} further improves the complexity to (nondeterministic) $O(n )$, i.e.,  linear space. 

%The connection between compression and word equations was first observed by Plandowski and Rytter \cite{PR98}. %, who showed that a length-minimal solution of size N has a compressed representation
%of size poly(n, log N). 
\OMIT{
	Essentially, the constraint language  $\strline[\replaceall]$ studied in this paper is word equations where the $\replaceall$ functions, which subsume the concatenation operation, are used. However, the additional straight-line restrictions are imposed.  
}

% TL: length constraints are not the main focus 
\OMIT{
Regarding the extension with length constraints, it is still a long-standing
open problem whether word equations with length constraints is decidable, though
it is known that letter-counting (e.g. counting the number of occurrences of 0s
and 1s separately) yields undecidability \cite{buchi}. It was shown in
\cite{LB16} that the length constraints (in fact, letter-counting) can be
added to the subclass of $\strline[\replaceall]$ where the pattern/replacement 
are constants, while preserving decidability. In contrast, if we allow 
variables on the replacement parameters of formulas in $\strline[\replaceall]$,
we can easily encode the Hilbert's 10th problem with length (integer) 
constraints. 
}

%In fact, this undecidability holds even if we use the unary
%alphabet $\Sigma = \{a\}$, and that the pattern string is
%always fixed to the letter $a$.

%Solving word equation was an intriguing problem since the beginning of computer science, investigated
%initially due to its ties to Hilbert’s 10th problem. Initially it was conjectured that this
%problem is undecidable, which was disproved by Makanin [10]. At the beginning little attention
%was given to computational complexity of Makanin’s algorithm and the problem itself; these questions
%were reinvestigated in the ’90 [6, 18, 9], culminating in the EXPSPACE implementation of
%Makanin’s algorithm by Gutiérrez [5].


%\cite{J17}
%Word equations in linear space
%
%Word equations are an important problem on the intersection of formal languages and algebra. Given two sequences consisting of letters and variables we are to decide whether there is a substitution for the variables that turns this equation into true equality of strings. The computational complexity of this problem remains unknown, with the best lower and upper bounds being NP and PSPACE. Recently, a novel technique of recompression was applied to this problem, simplifying the known proofs and lowering the space complexity to (nondeterministic) O(n log n). In this paper we show that word equations are in nondeterministic linear space, thus the language of satisfiable word equations is context-sensitive. We use the known recompression-based algorithm and additionally employ Huffman coding for letters. The proof, however, uses analysis of how the fragments of the equation depend on each other as well as a new strategy for nondeterministic choices of the algorithm, which uses several new ideas to limit the space occupied by the letters.


\OMIT{
	%A Decision Procedure for String Logic with Equations, Regular Membership and Length Constraints 
	Le \cite{L16} considered the satisfiability problem for string logic with word equations, regular membership and Presburger constraints over length functions. %The difficulty comes from multiple occurrences of string variables making state-of-the-art algorithms non-terminating. Our main contribution is to 
	He showed that the satisfiability problem in a fragment where no string variable occurs more than twice in an equation is decidable. 
	%In particular, he proposed a semi-decision procedure for arbitrary string formulae with word equations, regular membership and length functions, and showed that the algorithm always terminates for the aforementioned decidable fragment, with a complexity analysis. 
	This work is largely distant from ours, as $\replaceall$ was not addressed. However, we mention that the fragment considered by Le allows Presburger constraints over length functions.
	%The essence of our procedure is an algorithm to enumerate an equivalent set of solvable disjuncts for the formula. We further show that the algorithm always terminates for the aforementioned decidable fragment. Finally, we provide a complexity analysis of our decision procedure to prove that it runs, in the worst case, in factorial time.
	
	%In \cite{BTV09} the authors discussed the problem of path feasibility for programs manipulating strings using a collection of standard string library functions. They prove results on the complexity of this problem, including its undecidability in the general case and decidability of some special cases. \tl{how would it connect to ours?}
}


\OMIT{

The $\replaceall$ function can be seen as a special, yet expressive, string transformation function, aka string transducer. From this viewpoint, the closest work is~\cite{LB16}, which we discuss extensively in the introduction. Here, we discuss two further 
%the $\replaceall$ function is also related to two 
recent transducer models: streaming string transducers \cite{AC10} and symbolic transducers \cite{symbolic-transducer}. 

A streaming string transducer is a finite state machine where  a finite set of string variables are used to store the intermediate results for output. The $\replaceall(x, e, y)$ term can be modelled by an extension of streaming string transducers \emph{with parameters}, that is, a streaming string transducer which reads an input string (interpreted as the value of $x$), uses $y$ as a free string variable which is presumed to be read-only, and updates a string variable $z$, which stores the computation result, by a string term which may involve $y$. Nevertheless, to the best of our knowledge, this extension of streaming string transducers has not been investigated so far. 

Symbolic transducers are an extension of Mealy machine to infinite alphabets by using a variable $cur$ to represent the symbol in the current position, and replacing the input and output letters in transitions with unary predicates $\varphi(cur)$ and terms involving $cur$ respectively. Symbolic transducers can model $\replaceall$ functions \emph{when the third parameter is a constant}. Inspired by symbolic transducers, it is perhaps an interesting future work to consider an extension of the $\replaceall$ function by allowing predicates as patterns. %to sequences of numerical values. 
For instance, one may consider the term $\replaceall(x, cur \equiv 0 \bmod 2, y)$ which replaces every even number in $x$ with $y$. %This, however, is not addressed in the current paper. 

Finally, the $\replaceall$ function is related to Array Folds Logic introduced by Daca et al \cite{DHK16}. The authors considered an extension of the quantifier-free theory of integer arrays with counting. The main feature of the logic is the \emph{fold} terms, borrowed from the folding concept in functional programming languages. Intuitively, a fold term applies a function to every element of the array to compute an output. If strings are treated as arrays over a finite domain (the alphabet), the $\replaceall$ function can be seen as a fold term. Nevertheless, the $\replaceall$ function goes beyond the fold terms considered in \cite{DHK16}, since it outputs a string (an array), instead of an integer. Therefore, the results in \cite{DHK16} cannot be applied to our setting.
}

\paragraph{Practical Solvers}
A large amount of recent work develops practical string solvers
including  Kaluza~\cite{Berkeley-JavaScript}, Hampi~\cite{HAMPI}, 
Z3-str~\cite{Z3-str}, CVC4~\cite{cvc4}, Stranger~\cite{YABI14}, Norn~\cite{Abdulla14}, S3 and S3P~\cite{S3,TCJ16},  FAT~\cite{Abdulla17}, and SLOTH~\cite{HJLRV18}.
%Among them, only Stranger, S3, and S3P support $\replaceall$.  

%String solvers that support concatenations and the replace-all operator are available. \cite{BTV09,TCJ14,YABI14,S3}

%\cite{BTV09} considered an efficient finite model finding method for string constraints. They develop a two-tier finite model finding procedure. First, an integer abstraction of string constraints are passed to an SMT (Satisfiability Modulo Theories) solver. The abstraction is either unsatisfiable, or the solver produces a model that fixes lengths of enough strings to reduce the entire problem to be finite domain. The resulting fixed-length string constraints are then solved in a second phase. 

%We implemented the procedure in a symbolic execution framework, report on the encouraging results and discuss directions for improving the method further.


In the Stranger tool, %Verifying string manipulating programs is a crucial problem in computer security. String operations are used extensively within web applications to manipulate user input, and their erroneous use is the most common cause of security vulnerabilities in web applications. We 
an automata-based approach was provided for symbolic analysis of PHP programs, where two different semantics $\replaceall$ were considered, namely, the leftmost and longest matching as well as the leftmost and shortest matching. Nevertheless, they focused on the abstract-interpretation based analysis of PHP programs and provided an \emph{over-approximation} of all the possible values of the string variables at each program point. Therefore, their string constraint solving algorithm is \emph{not} an exact decision procedure. In contrast, we provided a decision procedure for the straight-line fragment with the rather general $\replaceall$ function, where the pattern parameter can be arbitrary regular expressions and the replacement parameter can be variables. In the latter case,  we consider the leftmost and longest semantics mainly for simplicity, and the decision procedure can be adapted to the leftmost and shortest semantics easily.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hide{
	For the string operations, the authors focus on two common ones: concatenation and replacement. The latter is close to---but not the same as---the $\replaceall$ function considered in this paper. However, in this paper, Yu et al provided   an \emph{over-approximation} of more %restricted replace 
	commonly used semantics, i.e., the longest match and first match semantics. 
	%
	%\cite{SMV12} translating regular expression matching into transducer. 
	%
	They use deterministic finite automata (DFAs) to represent possible values of string variables. Using forward reachability analysis we compute an over-approximation of all possible values that string variables can take at each program point. They also implemented Stranger, an automata-based string analysis tool, with experiments. In general, this is essentially an abstract interpretation based approach.  In comparison, our algorithm is also automata-based, but we work on a semantics of $\replaceall$, but not its approximation. \tl{more need to be said here}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Intersecting these with a given attack pattern yields the potential attack strings if the program is vulnerable. Based on the presented techniques, we have implemented Stranger, an automata-based string analysis tool for detecting string-related security vulnerabilities in PHP applications. We evaluated Stranger on several open-source Web applications including one with 350,000+ lines of code. Stranger is able to detect known/unknown vulnerabilities, and, after inserting proper sanitization routines, prove the absence of vulnerabilities with respect to given attack patterns.


The S3 and S3P tools also support the $\replaceall$ function, where some
progressive searching strategies were provided to deal with the non-termination
problem caused by the recursively defined string operations (of which 
$\replaceall$ is a special case). Nevertheless, the solvers are 
incomplete as reasoning about unbounded strings defined recursively is in 
general an undecidable problem.


%, the authors present S3 (which stands for Symbolic String Solver), a new symbolic string solver.
%The constraint language covers all the main string operations including the replace-all function. The authors 
%provided algorithms which make use of a symbolic representation so that membership in a set defined by a regular expression can be encoded as string equations. 

%To amplify this point, let us now state some statistics from a comprehensive
%study of practical JavaScript applications [28]. Constraints
%arising from the applications have an average (per benchmark
%query) of 63 JavaScript string operations, while the remaining
%are boolean, logical and arithmetic constraints. The largest fraction
%are for operations like indexOf, length (78%). A significant
%fraction of the operations, including substring (5%), replace
%(8%), and split, match (1%). Of the match, split and
%replace operations, 31% are based on regular expressions. Operations
%such as replace and split give rise to new strings
%from the original ones, thereby giving rise to constraints involving
%multiple string variables.



%. The algorithm first makes use of a symbolic representation
%so that membership in a set defined by a regular expression
%can be encoded as string equations. Secondly, there is a constraint based
%generation of instances from these symbolic expressions so
%that the total number of instances can be limited. 
%
%We evaluate S3 on a well-known set of practical benchmarks, demonstrating both
%its robustness (more definitive answers) and its efficiency (about 20
%times faster) against the state-of-the-art.



\hide{
	%Progressive Reasoning over Recursively-Defined Strings
	\cite{TCJ16} 
	Trinh et al considered %the problem of reasoning over an expressive constraint language for unbounded strings. 
	%In particular, they considered 
	recursively defined string functions, a very expressive way to define functions manipulating strings. This includes a recursive definition of the replace-all function considered in this paper\footnote{\cite{TCJ16} used the notation \textbf{replace}}. The authors argue that ``the difficulty comes from ``recursively defined" functions such as replace, making state-of-the-art algorithms non-terminating." They proposed a progressive search algorithm, %to not only mitigate the problem of non-terminating reasoning but also guide the search towards a “minimal solution” when the input formula is in fact satisfiable. We have 
	implemented within the state-of-the-art Z3 framework, with experimental evaluations. The algorithm is genetic and  applicable to all recursively defined string functions, but it is doomed to be incomplete as reasoning about unbounded strings defined recursively is in general an undecidable problem.   
	
	The focus of our work is on the fundamental issue of decidability, and this is complementary to the work. Our result may be considered a completeness guarantee for existing string solver. 
}

%Importantly, we have enabled conflict clause learning for string theory so that our solver can be used effectively in the setting of program verification. Finally, our experimental evaluation shows leadership in a large benchmark suite, and a first deployment for another benchmark suite which requires reasoning about string formulas of a class that has not been solved before.



%===========================================================
%
%\subsection*{Other related work}




%Symbolic Finite State Transducers:
%Algorithms and Applications

%
%Finite automata and finite transducers are used in a wide
%range of applications in software engineering, from regular
%expressions to specification languages. We extend these
%classic objects with symbolic alphabets represented as parametric
%theories. Admitting potentially infinite alphabets
%makes this representation strictly more general and succinct
%than classical finite transducers and automata over strings.
%Despite this, the main operations, including composition,
%checking that a transducer is single-valued, and equivalence
%checking for single-valued symbolic finite transducers are
%effective given a decision procedure for the background theory.
%We provide novel algorithms for these operations and
%extend composition to symbolic transducers augmented with
%registers. Our base algorithms are unusual in that they are
%nonconstructive, therefore, we also supply a separate model
%generation algorithm that can quickly find counterexamples
%in the case two symbolic finite transducers are not
%equivalent. The algorithms give rise to a complete decidable
%algebra of symbolic transducers. Unlike previous work, we
%do not need any syntactic restriction of the formulas on the
%transitions, only a decision procedure. In practice we leverage
%recent advances in satisfiability modulo theory (SMT)
%solvers. We demonstrate our techniques on four case studies,
%covering a wide range of applications. Our techniques
%can synthesize string pre-images in excess of 8, 000 bytes
%in roughly a minute, and we find that our new encodings
%significantly outperform previous techniques in succinctness
%and speed of analysis
% 

